Breaking the Loop: Recursive Proofs for Coinductive Predicates in Fibrations

The purpose of this paper is to develop and study recursive proofs of coinductive predicates. Such recursive proofs allow one to discover proof goals in the construction of a proof of a coinductive predicate, while still allowing the use of up-to techniques. This approach lifts the burden to guess invariants, like bisimulation relations, beforehand. Rather, they allow one to start with the sought-after proof goal and develop the proof from there until a point is reached, at which the proof can be closed through a recursion step. Proofs given in this way are both easier to construct and to understand, similarly to proofs given in cyclic proof systems or by appealing parameterised coinduction. In this paper, we develop a framework for recursive proofs of coinductive predicates that are given through fibrational predicate liftings. This framework is built on the so-called later modality, which has made its appearance in type theoretic settings before. In particular, we show the soundness and completeness of recursive proofs, we prove that compatible up-to techniques can be used as inference rules in recursive proofs, and provide some illustrating examples.

==> content/proof-system.tex <==
\section{Proof Rules}
\label{sec:proof-system}

\begin{equation*}
  \AxiomC{}
  \UnaryInfC{$\bparens{\later \ch{\Phi}}^{\sigma} \to \ch{\Phi}^\sigma$}
  \RightLabel{next}
  \UnaryInfC{$\bparens{\later \ch{\Phi}}^{\later \sigma} \to \ch{\Phi}^\sigma$}
  \RightLabel{\lemRef{later-exp-distr}}
  \UnaryInfC{$\later \bparens{\ch{\Phi}^\sigma} \to \ch{\Phi}^\sigma$}
  \RightLabel{Löb}
  \UnaryInfC{$\T \to \ch{\Phi}^\sigma$}
  \DisplayProof
\end{equation*}
